SIGNeRF: Scene Integrated Generation for Neural Radiance Fields

Advances in image diffusion models have recently led to notable improvements in the generation of high-quality images. In combination with Neural Radiance Fields (NeRFs), they enabled new opportunities in 3D generation. However, most generative 3D approaches are object-centric and applying them to editing existing photorealistic scenes is not trivial. We propose SIGNeRF, a novel approach for fast and controllable NeRF scene editing and scene-integrated object generation. A new generative update strategy ensures 3D consistency across the edited images, without requiring iterative optimization. We find that depth-conditioned diffusion models inherently possess the capability to generate 3D consistent views by requesting a grid of images instead of single views. Based on these insights, we introduce a multi-view reference sheet of modified images. Our method updates an image collection consistently based on the reference sheet and refines the original NeRF with the newly generated image set in one go. By exploiting the depth conditioning mechanism of the image diffusion model, we gain fine control over the spatial location of the edit and enforce shape guidance by a selected region or an external mesh.

==> todo.tex <==
What needs to happen until Saturday 9am 
Upload before deadline

# Schreiben TODO
- Kürzen aller Texte
- Introduction is ok 
- Result und Method kürzen 
- Was schreiben in Method 
    - Reference Geschichte 
- 

# Teaser 
Wie arbeit + Refrence sheet (Frage ob tauschen mit anderen Szenen -> nein) 

# Pipeline 
Bild machen 
Original NeRF reduzieren in größe 
Loop darstellen der alle Daten ersetzt 
Eher abstrahieren 

# Experimenten 
Wie sieht aus ohne Reference Sheet ohne COntrolnet mit und ohne (Supplementary oder Appendix)
Revison of Reference Sheet maybe (Supplementary oder Appendix)
(Selection modes entweder zusammen oder kürzen)

Ergebnisse 
Qualitative Szene die besser funktioniert 
Object editing und generation in einer 

Ergbnisse SDXL durchlaufen lassen 

Vergelich
Panda Szene und die Hut Szene 


Tabel durchlaufen lassen für SDXL 
Background Preservation fixen 


Limitations -> schreiben als graphisch zeigen (wenn dann sublementary) 
Object Centric 



Scheduler Zero123++

